Transactions on Red-black and AVL trees in NVRAM

Byte-addressable non-volatile memory (NVRAM) supports persistent storage with low latency and high bandwidth. Complex data structures in it ought to be updated transactionally, so that they remain recoverable at all times. Traditional database technologies such as keeping a separate log, a journal, or shadow data work on a coarse-grained level, where the whole transaction is made visible using a final atomic update operation. These methods typically need significant additional space overhead and induce non-trivial overhead for log pruning, state maintenance, and resource (de-)allocation. Thus, they are not necessarily the best choice for NVRAM, which supports fine-grained, byte-addressable access. We present a generic transaction mechanism to update dynamic complex data structures `in-place' with a constant memory overhead. It is independent of the size of the data structure. We demonstrate and evaluate our approach on Red-Black Trees and AVL Trees with a redo log of constant size (4 resp. 2 cache lines). The redo log guarantees that each accepted (started) transaction is executed eventually despite arbitrary many system crashes and recoveries in the meantime. We update complex data structures in local and remote NVRAM providing exactly once semantics and durable linearizability for multi-reader single-writer access. To persist data, we use the available processor instructions for NVRAM in the local case and remote direct memory access (RDMA) combined with a software agent in the remote case.

==> avl-insert-sm.tex <==
\begin{tikzpicture}
  \begin{scope}[>=stealth,x=2.5mm,y=2.5mm]
  \clip (-1.6,17.7) rectangle (13.6,37.3);
  %%\sffamily%%
  \smaller\smaller\smaller
  \let\sizebox\relax
  \newlength{\sizebox}\setlength{\sizebox}{2.8mm}

  \tikzstyle{box}=[draw,circle,inner sep=0pt,align=center,text width=1.5\sizebox,minimum size=1.8\sizebox,text height=1.5ex,text depth=.25ex]

  %% states
  \node[box,double] (clean) at (5,37) {C};
  \node[box,fill=gray!30!white] (A1) at (0,35.6) {A1};
  \node[box,fill=gray!30!white] (A2) at (3.5,33.6) {A2};
  %%\node[box,fill=gray!30!white] (A3) at (9,31) {A3};
  \node[box,fill=gray!30!white] (A4) at (3.5,30.4) {A4};
  %%\node[box,fill=gray!30!white] (A5) at (2,31) {A5};
  %%\node[box,fill=gray!30!white] (A6) at (2,24) {A6};
  \node[box,fill=gray!30!white] (A7) at (0,26.2) {A7};
  \node[box,fill=gray!30!white] (A8) at (0,23) {A8};
  \node[box,fill=gray!30!white] (A9) at (4,19.8) {A9};
  \node[box,fill=gray!30!white] (A10) at (4,26.2) {A10};
  \node[box,fill=gray!30!white] (A11) at (0,19.8) {A11};
  \node[box,fill=gray!30!white] (A12) at (4,23) {A12};
  \node[box,fill=gray!30!white] (A13) at (8,23) {A13};
  \node[box,fill=gray!30!white] (A14) at (8,26.2) {A14};


  \node[box,fill=gray!30!white] (A15) at (8.5,29.4) {A15};
  \node[box,fill=gray!30!white] (A16) at (8,19.8) {A16};
  \node[box,fill=gray!30!white] (A17) at (12,19.8) {A17};
  \node[box,fill=gray!30!white] (A18) at (12,23) {A18};
  \node[box,fill=gray!30!white] (A19) at (12,26.2) {A19};
  \node[box,fill=gray!30!white] (A20) at (12,29.4) {A20};

  \node[box,fill=gray!30!white] (A21) at (12,32.6)  {A21};
  \node[box,fill=gray!30!white] (A22) at (6.5,33.6)  {A22};
  \node[box,fill=gray!30!white] (A23) at (11,35.6) {A23};
  \node[box,fill=gray!30!white] (A24) at (8,37) {A24};

  \node[box,fill=gray!30!white] (A25) at (0,32.6) {A25};
  \node[box,fill=gray!30!white] (A26) at (0,29.4) {A26};

  %% transitions
  \sffamily%%

  \draw[dashed,->] (clean) to[bend left=10] (A1);
  \draw[->] (clean) -- (A2);

  \draw[->] (A1) to[bend left=10] node[sloped,pos=0.5,above=2pt] {new}  (clean); % insert new node

  \draw[dashed,->] (A2) -- (A25); %% init variables

  \draw[->] (A4) to[out=60,in=-90] (clean);  % insert new node
  \draw[->] (A4) -- (A7); % insert new node

  \draw[dashed,->] (A7) -- (A8);
  \draw[dashed,->] (A7) -- (A10);

  \draw[dashed,->] (A8) -- (A11);

  \draw[dashed,->] (A9) -- (A12);

  \draw[dashed,->] (A10) -- (A13);
  \draw[dashed,->] (A10) -- (A22);
  \draw[dashed,->] (A10) to[out=45,in=-120] (A23);

  \draw[->] (A11) -- (A9);

  \draw[dashed,->] (A12) -- (A8);
  \draw[dashed,->] (A12) -- (A10);

  \draw[dashed,->] (A13) -- (A14);
  \draw[dashed,->] (A13) -- (A16);

  \draw[->] (A14) -- (A15);

  \draw[->] (A15) -- (A22) node[sloped,pos=0.6,above=1pt] {rot}; %% rotation
  \draw[->] (A15) -- (A23) node[sloped,pos=0.3,below=1pt] {rot};

  \draw[dashed,->] (A16) -- (A17);

  \draw[->] (A17) -- (A18);

  \draw[dashed,->] (A18) -- (A19);

  \draw[->] (A19) -- (A20) node[sloped,pos=0.4,above=1pt] {rot}; %% rotation

  \draw[dashed,->] (A20) -- (A21);

  \draw[->] (A21) -- (A22) node[sloped,pos=0.7,above=1pt] {rot}; %% rotation
  \draw[->] (A21) -- (A23) node[sloped,pos=0.5,above=3pt] {rot}; %% rotation

  \draw[dashed,->] (A22) -- (clean);

  \draw[dashed,->] (A23) -- (A24);

  \draw[->] (A24) -- (clean);

  \draw[dashed, ->] (A25) -- (A26);

  \draw[dashed,->] (A26) -- (A4);

  \end{scope}
\end{tikzpicture}


==> avl-remove-sm.tex <==
\begin{tikzpicture}
  \begin{scope}[>=stealth,x=2.5mm,y=2.5mm]
  \clip (-1.6,18.0) rectangle (18.5,37.9);
  %%\sffamily%%
  \smaller\smaller\smaller
  \let\sizebox\relax
  \newlength{\sizebox}\setlength{\sizebox}{2.8mm}

  \tikzstyle{box}=[draw,circle,inner sep=0pt,align=center,text width=1.5\sizebox,minimum size=1.8\sizebox,text height=1.5ex,text depth=.25ex]

  %% states
%  \node[box,double] (clean) at (6.0,30) {C};
%  \node[box,fill=gray!30!white] (R1) at (4.0,34.5) {R1};
%  \node[box,fill=gray!30!white] (R2) at (0.0,34) {R2};
%  \node[box,fill=gray!30!white] (R3) at (2.7,31) {R3};
%  \node[box,fill=gray!30!white] (R4) at (3.9,28) {R4};
%  \node[box,fill=gray!30!white] (R5) at (2.2,26) {R5};
%  \node[box,fill=gray!30!white] (R6) at (4.5,25) {R6};
%  \node[box,fill=gray!30!white] (R7) at (0,31) {R7};
%  \node[box,fill=gray!30!white] (R8) at (0.0,27) {R8};
%  \node[box,fill=gray!30!white] (R9) at (1,24) {R9};
%  \node[box,fill=gray!30!white] (R10) at (2.5,21) {R10};
%  \node[box,fill=gray!30!white] (R11) at (0,20) {R11};
%  \node[box,fill=gray!30!white] (R12) at (0,17.0) {R12};
%  \node[box,fill=gray!30!white] (R13) at (3.0,18) {R13};
%  \node[box,fill=gray!30!white] (R14) at (5.5,17) {R14};
%
%  \node[box,fill=gray!30!white] (R15) at (11.0,31) {R15};
%  \node[box,fill=gray!30!white] (R16) at (8.0,26) {R16};
%  \node[box,fill=gray!30!white] (R17) at (7.3,20.0) {R17};
%  \node[box,fill=gray!30!white] (R18) at (14.5,17) {R18};
%  \node[box,fill=gray!30!white] (R19) at (14.2,22.2) {R19};
%  \node[box,fill=gray!30!white] (R20) at (5.0,22) {R20};
%
%  \node[box,fill=gray!30!white] (R21) at (12.0,20)  {R21};
%  \node[box,fill=gray!30!white] (R22) at (13.0,25)  {R22};
%  \node[box,fill=gray!30!white] (R23) at (11.1,27) {R23};
%  \node[box,fill=gray!30!white] (R24) at (16.5,33.5) {R24};
%
%  \node[box,fill=gray!30!white] (R25) at (12.5,34.0) {R25};
%  \node[box,fill=gray!30!white] (R26) at (8.3,34.5) {R26};
%
%  \node[box,fill=gray!30!white] (R27) at (8.3,31) {R27};
%  \node[box,fill=gray!30!white] (R28) at (11.2,23.2) {R28};
%  \node[box,fill=gray!30!white] (R29) at (8.5,22.6) {R29};
%  \node[box,fill=gray!30!white] (R30) at (16.2,24) {R30};
%  \node[box,fill=gray!30!white] (R31) at (14.0,27) {R31};
%  \node[box,fill=gray!30!white] (R32) at (16.2,27) {R32};
%  \node[box,fill=gray!30!white] (R33) at (17.2,30) {R33};
%  \node[box,fill=gray!30!white] (R34) at (14.0,30) {R34};

  \node[box,double] (clean) at (7.0,30) {C};
  \node[box,fill=gray!30!white] (R1) at (3.5,36.4) {R1};
  \node[box,fill=gray!30!white] (R2) at (0.0,36.4) {R2};
  \node[box,fill=gray!30!white] (R3) at (3.5,33.2) {R3};
  \node[box,fill=gray!30!white] (R4) at (1.8,28.6) {R4};
  \node[box,fill=gray!30!white] (R5) at (4.5,30.1) {R5};
  \node[box,fill=gray!30!white] (R6) at (3.7,26.2) {R6};
  \node[box,fill=gray!30!white] (R7) at (0,33.2) {R7};
  \node[box,fill=gray!30!white] (R8) at (0,30) {R8};
  \node[box,fill=gray!30!white] (R9) at (0,26.8) {R9};
  \node[box,fill=gray!30!white] (R10) at (0,23.6) {R10};
  \node[box,fill=gray!30!white] (R11) at (0,20.4) {R11};
  \node[box,fill=gray!30!white] (R12) at (3.5,20.4) {R12};
  \node[box,fill=gray!30!white] (R13) at (3.5,23.6) {R13};
  \node[box,fill=gray!30!white] (R14) at (7,23.6) {R14};

  \node[box,fill=gray!30!white] (R15) at (10.5,30) {R15};
  \node[box,fill=gray!30!white] (R16) at (10.5,26.8) {R16};
  \node[box,fill=gray!30!white] (R17) at (7,20.4) {R17};
  \node[box,fill=gray!30!white] (R18) at (10.5,20.4) {R18};
  \node[box,fill=gray!30!white] (R19) at (14,20.4) {R19};
  \node[box,fill=gray!30!white] (R20) at (7.0,26.8) {R20};

  \node[box,fill=gray!30!white] (R21) at (10.5,23.6)  {R21};
  \node[box,fill=gray!30!white] (R22) at (16.2,25.3)  {R22};
  \node[box,fill=gray!30!white] (R23) at (14,30) {R23};
  \node[box,fill=gray!30!white] (R24) at (14,36.4) {R24};

  \node[box,fill=gray!30!white] (R25) at (10.5,36.4) {R25};
  \node[box,fill=gray!30!white] (R26) at (7.0,36.4) {R26};

  \node[box,fill=gray!30!white] (R27) at (10.5,33.2) {R27};
  \node[box,fill=gray!30!white] (R28) at (14,23.6) {R28};
  \node[box,fill=gray!30!white] (R29) at (14,26.8) {R29};
  \node[box,fill=gray!30!white] (R30) at (17.2,20.4) {R30};
  \node[box,fill=gray!30!white] (R31) at (14,33.2) {R31};
  \node[box,fill=gray!30!white] (R32) at (17.2,30) {R32};
  \node[box,fill=gray!30!white] (R33) at (17.2,33.2) {R33};
  \node[box,fill=gray!30!white] (R34) at (17.2,36.4) {R34};



  %% transitions
  \sffamily%%

  \draw[dashed,->] (clean) to[bend right=7] (R1);
  \draw[dashed,->] (clean) to[out=40,in=90,looseness=2.7] (clean);

  \draw[->] (R1) to[bend right=7] (clean);
  \draw[->] (R1) -- (R2);
  \draw[->] (R1) to[bend right=22] (R4);
  \draw[->] (R1) -- (R7);

  \draw[dashed,->] (R2) to[bend right=10] (R3);

  \draw[->] (R3) -- (clean);
  \draw[->] (R3) to[bend right=10] (R2);
  \draw[->] (R3) -- (R4);
  \draw[->] (R3) -- (R7);

  \draw[dashed,->] (R4) -- (R5);
  \draw[dashed,->] (R4) -- (R6);

  \draw[->] (R5) -- (R20);

  \draw[dashed,->] (R6) -- (R20);

  \draw[->] (R7) -- (R8);

  \draw[->] (R8) -- (R9);
  \draw[->] (R8) to[bend right=28] (R11);

  \draw[dashed,->] (R9) to[bend right=10] (R10);
  \draw[dashed,->] (R9) to[bend left=35] (R11);

  \draw[->] (R10) to[bend right=10] (R9);
  \draw[->] (R10) -- (R11);

  \draw[->] (R11) -- (R12);

  \draw[dashed,->] (R12) -- (R13);

  \draw[->] (R13) -- (R20);

  \draw[dashed,->] (R14) -- (R17);

  \draw[->] (R15) -- (R20);

  \draw[dashed,->] (R16) -- (R20);

  \draw[->] (R17) to[bend right=35] (clean); %%to[out=-30,in=30,looseness=2.6]
  \draw[->] (R17) -- (R18);
  \draw[->] (R17) to[bend left=30] (R20);

  \draw[dashed,->] (R18) -- (R19);
  \draw[dashed,->] (R18) to[bend right=30] (R30);
  \draw[dashed,->] (R18) -- (R21);

  \draw[->] (R19) -- (R22);

  \draw[dashed,->] (R20) -- (R14);
  \draw[dashed,->] (R20) -- (clean);

  \draw[->] (R21) -- (R28);

  \draw[dashed,->] (R22) -- (R23);

  \draw[->] (R23) -- (R15); %% rotation
  \draw[->] (R23) -- (R16);

  \draw[dashed,->] (R24) -- (R25);

  \draw[->] (R25) -- (R26); %% rotation

  \draw[dashed,->] (R26) -- (R27);

  \draw[->] (R27) -- (R15); %% rotation
  \draw[->] (R27) to[bend right=35] (R16);

  \draw[dashed,->] (R28) -- (R29);

  \draw[->] (R29) -- (R15); %% rotation
  \draw[->] (R29) -- (R16);

  \draw[dashed,->] (R30) to[out=82,in=-60,looseness=1.0] (R31);
  \draw[dashed,->] (R30) to[out=82,in=-74,looseness=1.0] (R32);
  \draw[dashed,->] (R30) to[out=82,in=-66,looseness=1.0] (R33);

  \draw[->] (R31) -- (R34);

  \draw[->] (R32) to[bend left=30] (R34);

  \draw[->] (R33) -- (R34);

  \draw[->] (R34) -- (R24);

  \end{scope}
\end{tikzpicture}


==> common.tex <==
  \tikzstyle{logbox}=[draw,inner sep=0pt,text width=5\sizebox,minimum width=6\sizebox,minimum height=6mm,text height=1.5ex,text depth=.25ex]
  \tikzstyle{logboxquad}=[draw,inner sep=0pt,text width=1.0\sizebox,minimum width=1.5\sizebox,minimum height=6mm,text height=1.5ex,text depth=.25ex]
  \tikzstyle{logbox2}=[draw,inner sep=0pt,text width=8\sizebox,minimum width=10\sizebox,minimum height=4mm,text height=1.5ex,text depth=.25ex]
  \tikzstyle{treebox2}=[draw,inner sep=0pt,text width=5\sizebox,minimum width=1.4*\sizebox,minimum height=6mm,text height=1.5ex,text depth=.25ex]
  \tikzstyle{cl}=[node distance=2.9mm]

  \tikzstyle{logbox2}=[draw,inner sep=0pt,text width=5\sizebox,minimum width=6\sizebox+0.3\pgflinewidth,minimum height=6mm,text height=1.5ex,text depth=.25ex]

\tikzset{
      iterators/.pic={
        \begin{scope}[scale=#1,every node/.style={scale=0.8*#1}]
          \begin{scope}[align=center, node distance=-\pgflinewidth]
            \node[logbox] (r0)                 {\larger\larger\emph{LastDir}};
            \node[logbox] (r1)  [right= of r0] {\larger\larger\emph{Dir}};
            \node[logbox] (r2)  [below= of r0] {\larger\larger\emph{Tp}};
            \node[logbox] (r3)  [right= of r2] {\larger\larger\emph{Grandp}};
            \node[logbox] (r4)  [below= of r2] {\larger\larger\emph{Parentp}};
            \node[logbox] (r5)  [right= of r4] {\larger\larger\emph{Qp}};
            \node[logbox] (r6)  [below= of r4] {\larger\larger\emph{Q2p}};
            \node[logbox] (r7)  [right= of r6] {\larger\larger\emph{Fp}};
          \end{scope}
          \draw[thick] (r0.north west) rectangle (r7.south east);
        \end{scope}
      }
    };

    \tikzset{
      redo/.pic={
        \begin{scope}[scale=#1,every node/.style={scale=0.8*#1}]
          \begin{scope}[align=center, node distance=-\pgflinewidth]
            \node[logbox] (r8)                  {\larger\larger\emph{TmpNode}};
            \node[logbox] (r9)  [right= of r8]  {\larger\larger\emph{Sp}};
            \node[logbox] (r10) [below= of r8]  {\larger\larger\emph{Dir'}};
            \node[logbox] (r11) [right= of r10] {\larger\larger\emph{Dir''}};
            \node[logbox] (r12) [below= of r10] {\larger\larger\emph{Savep}};
            \node[logbox] (r13) [right= of r12] {\larger\larger\emph{Savechldp}};
          \end{scope}
          \draw[thick] (r8.north west) rectangle (r13.south east);
        \end{scope}
      }
    };

    \tikzset{
      log/.pic={
        \begin{scope}[scale=#1,every node/.style={scale=0.8*#1}]
          \begin{scope}[align=center, node distance=-\pgflinewidth]
             \node[logbox,draw=none] (dummy) {};
             \node[logbox,minimum width=12\sizebox] (r14) [below= of dummy.north east]    {\larger\larger\emph{Key}};
             \node[logbox,minimum width=12\sizebox] (r15) [below= of r14] {\larger\larger\emph{Value}};
             \node[logbox] (r16) [below= of r15.south west,anchor=north west] {\larger\larger\emph{Root}};
             \node[logbox] (r17) [right= of r16] {}; %% \larger\larger\emph{Head}
          \end{scope}
          \draw[thick] (r14.north west) rectangle (r17.south east);
          \end{scope}
      }
    };

    %% tree allocator
    \tikzset{
      tree2/.pic={
        \begin{scope}[scale=#1,every node/.style={scale=0.8*#1}]
          \begin{scope}[align=center, node distance=-\pgflinewidth]
             \node[logbox,draw=none] (dummy) {};

             %% sample node layout
             \node[logbox,minimum width=12\sizebox] (d0)  [below left = 2.1cm and 1cm of dummy]   {\larger\larger\emph{Key}};
             \node[logbox,minimum width=12\sizebox] (d1) [below= of d0] {\larger\larger\emph{Value}};
             \node[logbox2] (d2) [below = -0.65\pgflinewidth of d1.south west,anchor=north west] {\larger\larger\emph{Left}};
             \node[logbox2] (d3) [right =  of d2] {\larger\larger\emph{Right}};
             \node[logbox2] (d4) [below = -0.65\pgflinewidth of d2] {\larger\larger\emph{Up}};
             \node[logboxquad] (d5) [right= of d4] {\smaller\emph{Col}}; %% or
             \node[logboxquad] (d6) [right= of d5] {\smaller\emph{Dir}};
             \node[logboxquad] (d7) [right= of d6] {\smaller\emph{Bal}};


            \node[treebox2,node distance=20mm] (head)  [below= of dummy]      {\larger\larger\emph{Head}};
            \node[treebox2] (n0)    [right= of head]{\larger\larger\emph{n0}};
            \node[treebox2,cl] (n1) [right= of n0]  {\larger\larger\emph{n1}};
            \node[treebox2] (n2)    [right= of n1]  {\larger\larger\emph{n2}};
            \draw[thick] (head.north west) rectangle (n0.south east);
            \draw[thick] (n1.north west) rectangle (n2.south east);

            \node[treebox2,cl] (n3) [below= of head]  {\larger\larger\emph{n3}};
            \node[treebox2] (n4)  [right= of n3]  {\larger\larger\emph{n4}};
            \node[treebox2,cl] (n5)  [right= of n4]  {\larger\larger\emph{n5}};
            \node[treebox2] (n6)  [right= of n5]  {\larger\larger\emph{n6}};
            \draw[thick] (n3.north west) rectangle (n4.south east);
            \draw[thick] (n5.north west) rectangle (n6.south east);

            %% zoom animation
            \draw[densely dotted] (d0.north east) -- (n3.north west);
            \draw[densely dotted] (d7.south east) -- (n3.south west);

            \node[treebox2,cl] (n7)  [below= of n3]  {\larger\larger\emph{n7}};
            \node[treebox2] (n8)  [right= of n7]  {\larger\larger\emph{n8}};
            \node[treebox2,cl] (n9)  [right= of n8]  {\larger\larger\emph{n9}};
            \node[treebox2] (n10) [right= of n9]  {\larger\larger\emph{n10}};
            \draw[thick] (n7.north west) rectangle (n8.south east);
            \draw[thick] (n9.north west) rectangle (n10.south east);

            \node[treebox2,cl] (n11) [below= of n7] {\larger\larger\emph{n11}};
            \node[treebox2] (n12) [right= of n11]  {\larger\larger\emph{n12}};
            \node[treebox2,cl] (n13) [right= of n12] {\larger\larger\emph{n13}};
            \node[treebox2] (n14) [right= of n13] {\larger\larger\emph{n14}};
            \draw[thick] (n11.north west) rectangle (n12.south east);
            \draw[thick] (n13.north west) rectangle (n14.south east);

            \node[treebox2,cl] (n15) [below= of n11] {\larger\larger\emph{n15}};
            \node[treebox2] (n16) [right= of n15] {\larger\larger\emph{n16}};
            \node[treebox2,cl] (n17) [right= of n16] {\larger\larger\emph{n17}};
            \node[treebox2] (n18) [right= of n17] {\larger\larger\emph{n18}};
            \draw[thick] (n15.north west) rectangle (n16.south east);
            \draw[thick] (n17.north west) rectangle (n18.south east);

            \node[treebox2,cl] (n19) [below= of n15] {\larger\larger\emph{n19}};
            \node[treebox2] (n20) [right= of n19] {\larger\larger\emph{n20}};
            \node[treebox2,cl] (n21) [right= of n20] {\larger\larger\emph{n21}};
            \node[treebox2] (n22) [right= of n21] {\larger\larger\emph{\ldots}};
            \draw[thick] (n19.north west) rectangle (n20.south east);
            \draw[thick] (n21.north west) rectangle (n22.south east);

             {\larger\larger \node[node distance=4mm] (cacheline) [right= of n6.south east] {\textsf{Cache-}\\\textsf{lines}};}
             \draw[->,shorten >=1mm] (cacheline) to[bend right=13] (n2.north east);
             \draw[->,shorten >=1mm] (cacheline) to[bend left=13] (n10.east);
             \draw[->,shorten >=1mm] (cacheline) to[bend left=13] (n18.east);

          \end{scope}
        \end{scope}
      }
    };


==> fsm-insert2.tex <==
\begin{tikzpicture}
  \begin{scope}[>=stealth,x=2.5mm,y=2.5mm]
  \clip (-1.6,13.0) rectangle (15.8,37.3);
  %%\sffamily%%
  \smaller\smaller\smaller
  \let\sizebox\relax
  \newlength{\sizebox}\setlength{\sizebox}{2.8mm}

  \tikzstyle{box}=[draw,circle,inner sep=0pt,align=center,text width=1.5\sizebox,minimum size=1.8\sizebox,text height=1.5ex,text depth=.25ex]

  %% states
  \node[box,double] (clean) at (4,37) {C};
  \node[box,fill=gray!30!white] (A1) at (0,35) {A1};
  \node[box,fill=gray!30!white] (A2) at (5.5,34) {A2};
  \node[box,fill=gray!30!white] (A3) at (9,31) {A3};
  \node[box,fill=gray!30!white] (A4) at (12,27.5) {A4};
  \node[box,fill=gray!30!white] (A5) at (2,31) {A5};
  \node[box,fill=gray!30!white] (A6) at (2,24) {A6};
  \node[box,fill=gray!30!white] (A7) at (2,19) {A7};
  \node[box,fill=gray!30!white] (A8) at (5.5,16) {A8};
  \node[box,fill=gray!30!white] (A9) at (9,17) {A9};
  \node[box,fill=gray!30!white] (A10) at (5.5,28) {A10};
  \node[box,fill=gray!30!white] (A11) at (9,24) {A11};
  \node[box,fill=gray!30!white] (A12) at (5.5,20) {A12};
  \node[box,fill=gray!30!white] (A13) at (12,20) {A13};
  \node[box,fill=gray!30!white] (A14) at (12,34) {A14};

  %% transitions
  \sffamily%%

  \draw[dashed,->] (clean) to[bend left=10] (A1);
  \draw[dashed,->] (clean) -- (A2);

  \draw[->] (A1) to[bend left=10] node[sloped,midway,above=1pt] {new} (clean);

  \draw[->] (A2) -- (A5) node[sloped,pos=.4,above=1pt] {init};
  \draw[->] (A2) -- (A10) node[pos=0.2,right=1pt] {init};
  \draw[->] (A2) to[out=180,in=130,looseness=1.1] node[pos=0.4,sloped,above=1pt] {init} (A6);
  \draw[->] (A2) -- (A3) node[sloped,pos=.4,above=1pt] {init};
  \draw[->] (A2) to[out=170,in=160,looseness=1.5] node[sloped,pos=.3,above=1pt] {init} (A12);
  \draw[->] (A2) to[out=4,in=56,looseness=1.1] node[sloped,pos=.1,above=0.5pt] {init} (A13);

  %% \draw[->] (A4) -- (A12) node[midway] {add};
  \draw[->] (A4) -- (A10) node[sloped,pos=.3,above=1pt] {add};
  \draw[->] (A4) to[bend left=13] node[pos=0.15,sloped,above=1pt] {add} (A6);
  \draw[->] (A4) to[out=-100,in=20] node[sloped,pos=.15,above=1pt] {add} (A12);
  \draw[->] (A4) -- (A13) node[sloped,pos=.3,above=1pt] {add};

  \draw[->] (A5) -- (A10) node[sloped,midway,above=1pt] {color};
  \draw[->] (A5) -- (A6) node[sloped,midway,below=1pt] {color};
  \draw[->] (A5) to[bend left=2]  node[sloped,pos=0.2,above=1pt] {color} (A12);
  \draw[->] (A5) to[out=-130,in=-105,looseness=2.1]  node[sloped,above=1pt,pos=.3] {color} (A13);

  \draw[dashed, ->] (A10) -- (A11);

  \draw[dashed, ->] (A6) -- (A7);

  \draw[dashed, ->] (A3) -- (A4);
  \draw[dashed, ->] (A3) -- (A5);
  \draw[dashed, ->] (A3) -- (A10);
  \draw[dashed, ->] (A3) to[out=240,in=30,looseness=1.6] (A6);
  \draw[dashed, ->] (A3) to[out=-110,in=77,looseness=0.4] (A12);
  \draw[dashed, ->] (A3) to[out=-10,in=70,looseness=1.2] (A13);

  \draw[->] (A11) -- (A12) node[sloped,pos=0.3,above=1pt] {rot};
  \draw[->] (A11) -- (A13) node[sloped,midway,above=1pt] {rot};

  \draw[->] (A7) -- (A8) node[sloped,pos=0.4,below=1pt] {rot};

  \draw[->] (A9) -- (A12) node[sloped,midway,below=1pt] {rot};
  \draw[->] (A9) -- (A13) node[sloped,pos=0.4,below=1pt] {rot};

  \draw[dashed, ->] (A12) to[bend left=2] (A5);
  \draw[dashed, ->] (A12) -- (A10);
  \draw[dashed, ->] (A12) -- (A6);
  \draw[dashed, ->] (A12) to[out=70,in=-100,looseness=.4] (A3);
  \draw[dashed, ->] (A12) to[out=-150,in=-90,looseness=2.7] (A12);
  \draw[dashed, ->] (A12) -- (A13) node[midway,below=1pt] {descend};

  \draw[->] (A13) to[out=45,in=-63] node[sloped,above=1pt] {root} (A14);

  \draw[->] (A14) to[bend right=12] node[sloped,midway,above=1pt] {black} (clean);

  \draw[dashed, ->] (A8) -- (A9);

  \end{scope}
\end{tikzpicture}


==> fsm-remove3.tex <==
\begin{tikzpicture}[>=stealth,x=2.5mm,y=2.5mm]
  \clip (-3.5,13.0) rectangle (13.8,37.3);
  %% \sffamily %%
  \smaller\smaller\smaller
  \let\sizebox\relax
  \newlength{\sizebox}\setlength{\sizebox}{3.0mm}

  \tikzstyle{box}=[draw,circle,inner sep=0pt,align=center,text width=1.5\sizebox,minimum size=1.8\sizebox,text height=1.5ex,text depth=.25ex]

  % states
  \node[box,double] (clean) at (5,37) {C};
  \node[box,fill=gray!30!white] (r1) at (2,34) {R1};
  \node[box,fill=gray!30!white] (r2) at (7,32.5) {R2};
  \node[box,fill=gray!30!white] (r3) at (9.5,29) {R3};
  \node[box,fill=gray!30!white] (r4) at (0,29) {R4};
  \node[box,fill=gray!30!white] (r5) at (5,28) {R5};
  \node[box,fill=gray!30!white] (r6) at (2.5,24) {R6};
  \node[box,fill=gray!30!white] (r7) at (6,21) {R7};
  \node[box,fill=gray!30!white] (r8) at (-1,24) {R8};
  \node[box,fill=gray!30!white] (r9) at (-.5,20) {R9};
  \node[box,fill=gray!30!white] (r10) at (3.5,17) {R10};
  \node[box,fill=gray!30!white] (r11) at (7.5,18) {R11};
  \node[box,fill=gray!30!white] (r12) at (11,21) {R12};
  \node[box,fill=gray!30!white] (r13) at (11,25) {R13};
  \node[box,fill=gray!30!white] (r14) at (11.5,31.5) {R14};
  \node[box,fill=gray!30!white] (r15) at (9.5,35) {R15};

  %% transitions
  \sffamily

  \draw[->] (clean) -- node[right=3pt,pos=.6] {init} (r1);

  \draw[dashed,->] (r1)  to[out=150,in=90,looseness=2.7] node[midway,left=3pt] {descend}(r1) ;
  \draw[dashed,->] (r1) -- (r2) node[midway,sloped,above=2pt] {descend};
  \draw[dashed,->] (r1) to[bend left=10] node[sloped,below=1pt ] {descend} (r4);
  \draw[dashed,->] (r1) -- (r13) node[sloped,pos=0.5,above=1pt] {descend};

  \draw[->] (r14) -- (r15) node[pos=.5,right=1pt] {remove};

  \draw[->] (r15) -- (clean) node[sloped,pos=0.4,above=1pt] {root};

  \draw[dashed, ->] (r2) to[bend left=10] (r3);

  \draw[->] (r3) -- (r1) node[sloped,pos=.2,above=1pt] {rot};
  \draw[->] (r3) -- node[sloped,pos=.4,above=1pt] {rot} (r13);

  \draw[dashed, ->] (r4) to[bend left=10] (r1);
  \draw[dashed, ->] (r4) -- (r5);
  \draw[dashed, ->] (r4) -- (r8);
  \draw[dashed, ->] (r4) -- (r6);
  \draw[dashed, ->] (r4) to[bend right=10] (r12);
  \draw[dashed, ->] (r4) to[bend right=15] (r13);

  \draw[->] (r5) -- (r1) node[pos=.3,left=1pt] {flip};
  \draw[->] (r5) -- node[sloped,pos=.2,above=1pt] {flip} (r13);

  \draw[dashed, ->] (r8) -- (r9);

  \draw[->] (r9) -- (r10) node[sloped,pos=.4,above=1pt] {rot};

  \draw[dashed, ->] (r10) -- (r11);

  \draw[->] (r11) -- (r12) node[sloped,pos=.4,above=1pt] {rot};

  \draw[dashed, ->] (r6) -- (r7);

  \draw[->] (r7) -- node[sloped,pos=.3,above=1pt] {rot} (r12);

  \draw[->] (r12) to[out=-115,in=-140,looseness=2.4] node[pos=.45,sloped,above=1pt] {color} (r1);
  \draw[->] (r12) -- (r13) node[pos=.6,left=1pt] {color};

  \draw[dashed, ->] (r13) -- (r14);

\end{tikzpicture}

